Provable RL with Exogenous Distractors via Multistep Inverse Dynamics

Many real-world applications of reinforcement learning (RL) require the agent to deal with high-dimensional observations such as those generated from a megapixel camera. Prior work has addressed such problems with representation learning, through which the agent can provably extract endogenous, latent state information from raw observations and subsequently plan efficiently. However, such approaches can fail in the presence of temporally correlated noise in the observations, a phenomenon that is common in practice. We initiate the formal study of latent state discovery in the presence of such exogenous noise sources by proposing a new model, the Exogenous Block MDP (EX-BMDP), for rich observation RL. We start by establishing several negative results, by highlighting failure cases of prior representation learning based approaches. Then, we introduce the Predictive Path Elimination (PPE) algorithm, that learns a generalization of inverse dynamics and is provably sample and computationally efficient in EX-BMDPs when the endogenous state dynamics are near deterministic. The sample complexity of PPE depends polynomially on the size of the latent endogenous state space while not directly depending on the size of the observation space, nor the exogenous state space. We provide experiments on challenging exploration problems which show that our approach works empirically.

==> app_multi_step_genIK.tex <==
\section{Multistep GenIK}\label{sec:multi step gen IK}

\begin{algorithm}
\caption{$\algname(S_{UB}, \delta)$ Generalized Inverse Kinematics with Path Prediction and Elimination.}
\label{alg:genik_path_elim}
\setstretch{1.25}
\begin{algorithmic}[1] 
% \State {\bf Require:} $\delta>0,$ $S_{UB}$ an upper bound on the state space for each $h\in [H]$, set $N = 16(S_{UB}A)^2\log\rbr{\frac{|\Fcal|H(S_{UB}A)^2}{\delta}}$ samples.
\State Set $\Psi_1 = \{\bot\}$ and $N = 16(S_{UB}A)^2\log\rbr{\frac{|\Fcal|H(S_{UB}A)^2}{\delta}}$ \mycomment{$\bot$ denotes an empty path}
\For{$h=2,\ldots,H$}
% \State Define $\Psi^E_{h} = \Psi_{h-1} \times \Acal$ \Comment{Extended policy cover}
\State Define $\pts_h = \Psi_{h-1} \times \Acal$ as the set of one-step extension of paths in $\Psi_{h-1}$. \label{line:extension}
\State Collect a dataset $\Dcal$ of $N$ \emph{i.i.d.} tuples $(x_h,x_\tau, \pt)$ where $$\pt \sim \unf(\pts_h),\ \tau \sim \unf(H), x_\tau \sim \PP(x_\tau| v) \textit{ and } x_h \sim \PP(x_h \mid x_\tau, v)$$
\State Solve:
            $
            \hat{f}_{h} = \argmax_{f \in \Fcal} \sum_{(x, \pt) \in \Dcal} \ln f(a_\tau \mid x_h,x_\tau,\tau).  
            $ 
%\State Create a validation dataset $\cbr{(\pt_n,x_{h,n})}_{n=1}^N$ by acting with $\pt_n\sim \mu\sim Uniform(\Psi_{h})$ and observing $x_{h}$.
\For{$i \in \{1, \cdots, |\pts_h|\}$ and $j \in \{i+1, \cdots, |\pts_h|\}$}
        \State Let $t_d$ be the first time step in which paths $\pt_i,\pt_j$ disagree, hence $a_{t_d}^{(i)}\neq a_{t_d}^{(j)}$
        \State Collect a dataset $\Dcal_s$ of $N$ i.i.d. tuples $(x_h,x_{t_d},a_{t_d})$ by following $\nu \sim \unf(\cbr{\pt_i,\pt_j})$ 
        \State Calculate prediction gap:
            $$
           \widehat{\Delta}(i, j) = \frac{1}{N}\sum_{(x_h,x_{t_d},a_{t_d}) \in \Dcal_s} \abr{\hat{f}_h(a_{t_d}^{(i)} | x_h,x_{t_d},t_d ) - \hat{f}_h(a_{t_d}^{(j)} | x_h,x_{t_d},t_d)}.
            $$
        \State If $\widehat{\Delta}(i, j) \leq \frac{1}{S_{UB}A}$, then eliminate path $\pt_j$. \mycomment{$\pt_i$ and $\pt_j$ visit the same endogenous state.} \label{line:elimination}
    \EndFor
\State $\Psi_h$ is defined as the set of all paths in $\pts_h$ that have not been eliminated in~\pref{line:elimination}.
\EndFor
\end{algorithmic}
\end{algorithm}




